REAP: An Efficient Incentive Mechanism for Reconciling Aggregation Accuracy and Individual Privacy in Crowdsensing

Incentive mechanism plays a critical role in privacy-aware crowdsensing. Most previous studies on co-design of incentive mechanism and privacy preservation assume a trustworthy fusion center (FC). Very recent work has taken steps to relax the assumption on trustworthy FC and allows participatory users (PUs) to add well calibrated noise to their raw sensing data before reporting them, whereas the focus is on the equilibrium behavior of data subjects with binary data. Making a paradigm shift, this paper aim to quantify the privacy compensation for continuous data sensing while allowing FC to directly control PUs. There are two conflicting objectives in such scenario: FC desires better quality data in order to achieve higher aggregation accuracy whereas PUs prefer adding larger noise for higher privacy-preserving levels (PPLs). To achieve a good balance therein, we design an efficient incentive mechanism to REconcile FC's Aggregation accuracy and individual PU's data Privacy (REAP). Specifically, we adopt the celebrated notion of differential privacy to measure PUs' PPLs and quantify their impacts on FC's aggregation accuracy. Then, appealing to Contract Theory, we design an incentive mechanism to maximize FC's aggregation accuracy under a given budget. The proposed incentive mechanism offers different contracts to PUs with different privacy preferences, by which FC can directly control PUs. It can further overcome the information asymmetry, i.e., the FC typically does not know each PU's precise privacy preference. We derive closed-form solutions for the optimal contracts in both complete information and incomplete information scenarios. Further, the results are generalized to the continuous case where PUs' privacy preferences take values in a continuous domain. Extensive simulations are provided to validate the feasibility and advantages of our proposed incentive mechanism.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-siggraph.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-siggraph.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> Privacyandaccuracy.tex <==
\section{Relationship between Privacy \\and Accuracy}\label{section:relationship}
In this section, we first define the privacy and aggregation accuracy. Then, the quantitative relationship between the PPLs of individual PUs and the aggregation accuracy of FC is derived.

\subsection{Privacy Definition}
We adopt the celebrated notion of differential privacy \cite{dwork2008differential} to quantify individual PU's PPL. Informally, differential privacy guarantees that, after receiving the observation, the attackers cannot distinguish the neighboring input with high confidence. Here, neighboring relationship is an important concept in differential privacy. In this paper, we adopt the neighboring relationship for continuous value as follows:
\begin{definition}[$\gamma_i$-adjacency]\label{definition:adjacency}
Two continuous data $d_i$ and $d_i'$ are $\gamma_i$-adjacency, if $|d_i-d_i'|\leq \gamma_i$, where $\gamma_i$ is the range of PU $i$'s sensing data $d_i$.
\end{definition}
%In this adjacency definition, we adopt $1$-norm for the distance definition, while the standard differential privacy adopt Hamming distance \cite{dwork2006calibrating}.

Then, we can give the formal definition of differential privacy.
\begin{definition}[$\epsilon_i$-differential privacy \cite{le2014differentially}]\label{definition:dp}
A random algorithm $\{\mathcal{A}:R \rightarrow R|\mathcal{A}(d_i)=d_i+\eta_i\}$ achieves $\epsilon_i$-differential privacy, if for all pairs of $\gamma_i$-adjacency data $d_i$ and $d_i'$, and observation $d^{obs}$,
\begin{align*}
Pr[\mathcal{A}(d_i)=d^{obs}]\leq e^{\epsilon_i}Pr[\mathcal{A}(d_i')=d^{obs}].
\end{align*}
\end{definition}

Intuitively, PU $i$'s accurate sensing data can be either $d_i$ or $d_i'$ from an attacker's view. After adding noise $\eta_i$, both $d_i$ and $d_i'$ can result in $d^{obs}$ with certain probability. Thus, an attacker cannot distinguish PU $i$'s accurate sensing data with high confidence when he observe $d^{obs}$.

The Laplacian mechanism \cite{dwork2006calibrating} is the first and probably most widely used mechanism for achieving differential privacy, it satisfies $\epsilon_i$-differential privacy by calibrating the Laplacian noise parameter based on the following lemma:
\begin{lemma}
If the Laplacian mechanism is used, i.e., $\eta_i\sim Lap(0,b_i)$, we can achieve $\epsilon_i$-differential privacy if $b_i=\frac{\gamma_i}{\epsilon_i}$.
\end{lemma}

\subsection{Accuracy Definition}
To quantify the aggregation accuracy of the privacy preserving sensing data, we adopt the following accuracy definition.
\begin{definition}[$(\alpha,\delta)$-accuracy]
The aggregation $\hat{s}$ of privacy-preserving sensing data achieves $(\alpha,\delta)$-accuracy if
\begin{align*}
Pr[|\hat{s}-s|\geq\alpha] \leq 1-\delta,
\end{align*}
\end{definition}
where $s$ is the aggregation result of accurate sensing data.

Intuitively, this definition indicates that the aggregation error is larger than $\alpha$, with probability at most $1-\delta$. From estimation's perspective, $\alpha$ stands for confidence interval and $\delta$ stands for confidence level. Clearly, for a given confidence level, a smaller confidence interval means better aggregation accuracy. Thus, we can leverage the confidence interval $\alpha$ under a certain confidence level to measure the \emph{aggregation accuracy}, where a smaller $\alpha$ means better aggregation accuracy.

\subsection{From PU's PPL to FC's Aggregation Accuracy}
So far, we have defined individual PU's PPL and FC's aggregation accuracy. Then, we can derive the relationship between them as the following lemma:
\begin{lemma}\label{lemma:relationship}
For a given confidence level $\delta\leq1$, the aggregation accuracy $\alpha$ of the privacy-preserving sensing data can be found as
\begin{align}\label{formula:relationship}
\alpha = \frac{\sqrt{2}\gamma}{n\sqrt{1-\delta}}\sqrt{\sum_{i=1}^n\frac{1}{\epsilon_i^2}}.
\end{align}
\end{lemma}
where $\epsilon_i$ is PU $i$'s PPL, $n$ is the number of PUs, and $\gamma$ is the range of PUs' sensing data\footnote{Notice that the range of the sensing data should be the same for all PUs in a specific crowdsensing application, for example, the heart rate of a normal adult is always in the range $60\sim100$ bpm. Thus, all PUs' $\gamma_i$ should take the same value, i.e., $\gamma_i=\gamma,\forall\gamma_i$.}. The proof can be found in Appendix \ref{appendix:1}.
%The proof can be found in the appendix.









